FasterViT: Fast Vision Transformers with Hierarchical Attention

We design a new family of hybrid CNN-ViT neural networks, named FasterViT, with a focus on high image throughput for computer vision (CV) applications. FasterViT combines the benefits of fast local representation learning in CNNs and global modeling properties in ViT. Our newly introduced Hierarchical Attention (HAT) approach decomposes global self-attention with quadratic complexity into a multi-level attention with reduced computational costs. We benefit from efficient window-based self-attention. Each window has access to dedicated carrier tokens that participate in local and global representation learning. At a high level, global self-attentions enable the efficient cross-window communication at lower costs. FasterViT achieves a SOTA Pareto-front in terms of accuracy and image throughput. We have extensively validated its effectiveness on various CV tasks including classification, object detection and segmentation. We also show that HAT can be used as a plug-and-play module for existing networks and enhance them. We further demonstrate significantly faster and more accurate performance than competitive counterparts for images with high resolution. Code is available at https://github.com/NVlabs/FasterViT.

==> Tables/results_high_res.tex <==


% \begin{table}[t]
%     \caption{Quantitative comparison between higher resolution fine-tuning of FasterViT and Swin Transformer V2 networks. FasterViT is more accurate on average by 0.9\%, and faster by 2x.}
%     \label{tab:swin-v2-com}
    
%        \centering\resizebox{0.8\linewidth}{!}{
%     \begin{tabular}{l|cc|cccccc}
%               & \multicolumn{2}{c|}{Pretrain}  & \multicolumn{6}{c}{Finetune}  \\
%               & \multicolumn{2}{c|}{W8, I256}      & \multicolumn{2}{c}{W12, I384} & \multicolumn{2}{c}{W16, I512} & \multicolumn{2}{c}{W24, I768}\\
%              Model & acc & im/s &  acc & im/s & acc & im/s & acc & im/s\\
%               \toprule
%         SwinV2-T~\cite{liu2022swin} & 81.8 & 1674      & 83.2 & 573  & 83.8 & 168 & 84.2 & 72 \\     
%         SwinV2-S~\cite{liu2022swin} & 83.7 & \ \  633       &  84.8    &  338 &85.4 & 153 & - & -\\ 

%             \rowcolor{Gray}
%      \textbf{FasterViT-2} & \textbf{84.3} & \textbf{2500}      & \textbf{85.3} & \textbf{984}  &\textbf{85.5} & \textbf{489}  & \textbf{85.6} & \textbf{155} \\
% \midrule
%         SwinV2-B~\cite{liu2022swin} & 84.2 &\ \   499      &    85.1     &    251    & 85.6 & 115 & - & - \\
%     \rowcolor{Gray}
%           \textbf{FasterViT-4 256} & \textbf{85.3} &\ \  \textbf{653}          &   \textbf{86.0 }   &   \textbf{254}   & \textbf{86.1} & \textbf{133} & \textbf{86.0} & \textbf{44}\\

%      \bottomrule
    
%     \end{tabular} 
%     }

% \end{table}




%model 4, 512 -> 133, 448 -> 180, 256 -> 653
%model 3a, 512 -> 274, 448 -> 384


% old 
% \begin{table}[t]

%     \centering\resizebox{.8\linewidth}{!}{
%     \begin{tabular}{l|cc|cc}
%     \toprule
%               & \multicolumn{2}{c|}{\textbf{Pretrain}}  & \multicolumn{2}{c}{\textbf{Finetune}}  \\
%  \cmidrule{2-5} 
%               & \multicolumn{2}{c|}{W8, I256}      &  \multicolumn{2}{c}{W16, I512}  \\
%  \cmidrule{2-5} 
%              \textbf{Model} & Top-1 & img/sec &  Top-1 & img/sec  \\
%               \toprule
%               SwinV2-T~\cite{liu2022swin} & 81.8 & 1674    & 83.8 & 168 \\ 
%               SwinV2-S~\cite{liu2022swin} & 83.7 & 633    & 85.4 & 153 \\ 
%         SwinV2-B~\cite{liu2022swin} & 84.2 & 499    & 85.6 & 115 \\     \rowcolor{Gray}
%      \textbf{FasterViT-2} & \textbf{84.3} & \textbf{2500}      & \textbf{85.5} & \textbf{489} \\
%      \rowcolor{Gray}
%      \textbf{FasterViT-4} & \textbf{85.1} & \textbf{653}      & \textbf{85.9} & \textbf{180} \\
%      \bottomrule
    
%     \end{tabular} 
%     }
%         \caption{Quantitative comparison between higher resolution fine-tuning of FasterViT and Swin Transformer V2 networks.}
%     \label{tab:swin-v2-com}
% \end{table}

%     \centering\resizebox{.893\linewidth}{!}{
%     \begin{tabular}{l|cc|ccccccc}
%               & \multicolumn{2}{c|}{ImageNet - Pretrain 300 Epochs}  & \multicolumn{6}{c}{ImageNet - Finetune 30 Epochs}  \\
%               & \multicolumn{2}{c|}{I256}      & \multicolumn{2}{c}{I384} & \multicolumn{2}{c}{I512} & \multicolumn{2}{c}{I768} & \\
%              Model & Top-1 & img/sec &  Top-1 & img/sec & Top-1 & img/sec & Top-1 & img/sec & \\
%               \toprule
%         Swin Transformer V2-T & 81.8 & 1674      & 83.2 & 573  & 83.8 & 168 & 84.2 & 72 \\     \rowcolor{Gray}
%      \textbf{FasterViT-2} & \textbf{83.6} & \textbf{2367}      & \textbf{83.7} & \textbf{1045}  & \textbf{84.0} & \textbf{605} & \textbf{84.0} & \textbf{262} \\
%      \bottomrule
    
% % ImageNet* W8, I256 top-1 acc 81.7
% % W12, I384 top-1 acc 79.4/82.7
% % W16, I512 top-1 acc 77.2/83.0
% % W20, I640 top-1 acc 73.2/83.2
% % W24, I768
%     \end{tabular} 
%     }
% \end{table*}

% repeat with augmentations 
% 





% \begin{table}
%     \caption{Ablation study on the effectiveness of HAT as a plug-and-play module with Swin-T model for various CV tasks.}
%     \label{tab:abl_study_cmt}
% \centering
% \resizebox{0.8\linewidth}{!}{
% \footnotesize
% \setlength{\tabcolsep}{2.5pt}
% \begin{tabular}{l|c|cc|c}
% \hline
%  & \multicolumn{1}{c|}{ImageNet} & \multicolumn{2}{c|}{COCO} & \multicolumn{1}{c}{ADE20k} \\
%  & top-1   & AP$^\text{box}$ & AP$^\text{mask}$ & mIoU \\
% \hline
% Swin-T & 81.3 & 50.4 & 43.7 & 44.5 \\
% \rowcolor{Gray}
% \textbf{Swin-T + HAT}  & \textbf{81.7} & \textbf{50.9} & \textbf{44.3} & \textbf{45.4} \\

% \hline
% \end{tabular}
%   }
% %   \vspace{3pt}
% \end{table}


% 2048?

% 512, window 16, v1 -> 596
% 512, window 16, v2 -> 489

% post training ablations on v1 on 224, load original model and do tests:
% original model is 82.9 
% no upsample (propagation) 82.068
% no attention on CT 79.97
% no 1D positional bias (attention bias is still there) 52.25

% \begin{table}[t]
%     \caption{Quantitative comparison between higher resolution fine-tuning of FasterViT and Swin Transformer V2 networks.}
%     \label{tab:swin-v2-com}
%     \centering\resizebox{.99\linewidth}{!}{
%     \begin{tabular}{l|cc|cccc}
%     \toprule
%               & \multicolumn{2}{c|}{\textbf{Pretrain}}  & \multicolumn{4}{c}{\textbf{Finetune}}  \\
%  \cmidrule{2-7} 
%               & \multicolumn{2}{c|}{I256}      & \multicolumn{2}{c}{I384} & \multicolumn{2}{c}{I512}  \\
%  \cmidrule{2-7} 
%              \textbf{Model} & Top-1 & img/sec &  Top-1 & img/sec & Top-1 & img/sec  \\
%               \toprule
%         Swin Transformer V2-T~\cite{liu2022swin} & 81.8 & 1674      & 83.2 & 573  & 83.8 & 168 \\     \rowcolor{Gray}
%      \textbf{FasterViT-2} & \textbf{84.26} & \textbf{2500}      & \textbf{xx} & \textbf{1061}  & \textbf{84.41} & \textbf{592} \\
%      \bottomrule
    
% % ImageNet* W8, I256 top-1 acc 81.7
% % W12, I384 top-1 acc 79.4/82.7
% % W16, I512 top-1 acc 77.2/83.0
% % W20, I640 top-1 acc 73.2/83.2
% % W24, I768
%     \end{tabular} 
%     }
% \end{table}





% \begin{table*}[t]
%     \caption{Quantitative comparison between higher resolution fine-tuning of FasterViT and Swin Transformer V2 networks. The proposed FasterViT-2 has a better memory usage as 4 $\times$ higher number of batches can be used on average.}
%     \label{tab:swin-v2-com}
%     \centering\resizebox{.893\linewidth}{!}{
%     \begin{tabular}{l|cc|ccccccc}
%               & \multicolumn{2}{c|}{ImageNet - Pretrain 300 Epochs}  & \multicolumn{6}{c}{ImageNet - Finetune 30 Epochs}  \\
%               & \multicolumn{2}{c|}{I256}      & \multicolumn{2}{c}{I384} & \multicolumn{2}{c}{I512} & \multicolumn{2}{c}{I768} & \\
%              Model & Top-1 & img/sec &  Top-1 & img/sec & Top-1 & img/sec & Top-1 & img/sec & \\
%               \toprule
%         Swin Transformer V2-T & 81.8 & 1674      & 83.2 & 573  & 83.8 & 168 & 84.2 & 72 \\     \rowcolor{Gray}
%      \textbf{FasterViT-2} & \textbf{83.6} & \textbf{2367}      & \textbf{83.7} & \textbf{1045}  & \textbf{84.0} & \textbf{605} & \textbf{84.0} & \textbf{262} \\
%      \bottomrule
    
% % ImageNet* W8, I256 top-1 acc 81.7
% % W12, I384 top-1 acc 79.4/82.7
% % W16, I512 top-1 acc 77.2/83.0
% % W20, I640 top-1 acc 73.2/83.2
% % W24, I768
%     \end{tabular} 
%     }
% \end{table*}





==> Tables/results_segmentation.tex <==
% \begin{table}[t]
% \centering
% \caption{Semantic segmentation benchmarks \textbf{ADE20K} dataset~\cite{zhou2017scene} with UPerNet~\cite{xiao2018unified} and pre-trained FasterViT backbones. All model statistics are reported using a input test resolution of $512\times 512$. Throughput is measured in image/sec.}
% \label{tab:adek20kseg}
% \resizebox{1\linewidth}{!}{
% \footnotesize
% % \setlength{\tabcolsep}{2.5pt}
%   \begin{tabular}{lcccc}
%     \toprule
%     Model  & Throughput & FLOPs (G) & IoU(ss/ms) \\
%     \midrule	 
%     % DeiT-Small/16~\cite{touvron2021training}  & 52 & 1099  & 44.0\\
%     Swin-T~\cite{liu2021swin}  & 350 & 945 & 44.5/45.8\\
%     ConvNeXt-T~\cite{liu2022convnet}  & 363 & 939  & \quad-\  /46.7\\
%          \rowcolor{Gray}
%     \textbf{FasterViT-2}  & \textbf{377} & 974  & \textbf{47.2/48.4}\\
%     \midrule
%     % ResNet-101~\cite{he2016deep}  & 86 & 1029  & -/44.9\\
%     % Focal-T~\cite{yang2021focal}  & 62 & 998 & -&45.8\\
%     % Twins-SVT-S~\cite{chu2021twins}  & -  &  - & 46.2/47.1\\
%     Twins-SVT-B~\cite{chu2021twins}  & 204 &  - & 47.7/48.9\\
%     Swin-S~\cite{liu2021swin}  & 219 & 1038  & 47.6/49.5\\
%     ConvNeXt-S~\cite{liu2022convnet}  & 234 & 1027  &\quad-\  /49.6\\
%         \rowcolor{Gray}
%     \textbf{FasterViT-3}  & \textbf{254} & 1076  & \textbf{48.7/49.7}\\
%     \midrule
%     % Focal-S~\citep{yang2021focal}  & 85 & 1130 & 48.0\\
%     Twins-SVT-L~\cite{chu2021twins}  & 164 & -  & 48.8/50.2\\
%     Swin-B~\cite{liu2021swin}  & 172 & 1188  & 48.1/49.7\\
%     ConvNeXt-B~\cite{liu2022convnet}  & 189 & 1170  &\quad-\  /49.9\\
%     \rowcolor{Gray}
%     \textbf{FasterViT-4}  & \textbf{202} & 1290  & \textbf{49.1/50.3}\\
%     \bottomrule

%   \end{tabular} 
%   }
%     \label{tab:ade_segmentation}
% \end{table}

% \begin{wraptable}{r}{7.6cm}
% % \vspace{-0.5mm}
% \begin{minipage}{1.0\linewidth}
% \small
% \centering
% \resizebox{1.\linewidth}{!}{
% \setlength{\tabcolsep}{2.5pt}
%   \begin{tabular}{lcccc}
%     \toprule
%     Model  & Throughput & FLOPs (G) & IoU(ss/ms) \\
%     \midrule	 
%     % DeiT-Small/16~\cite{touvron2021training}  & 52 & 1099  & 44.0\\
%     Swin-T~\cite{liu2021swin}  & 350 & 945 & 44.5/45.8\\
%     ConvNeXt-T~\cite{liu2022convnet}  & 363 & 939  & \quad-\  /46.7\\
%          \rowcolor{Gray}
%     \textbf{FasterViT-2}  & \textbf{377} & 974  & \textbf{47.2/48.4}\\
%     \midrule
%     % ResNet-101~\cite{he2016deep}  & 86 & 1029  & -/44.9\\
%     % Focal-T~\cite{yang2021focal}  & 62 & 998 & -&45.8\\
%     % Twins-SVT-S~\cite{chu2021twins}  & -  &  - & 46.2/47.1\\
%     Twins-SVT-B~\cite{chu2021twins}  & 204 &  - & 47.7/48.9\\
%     Swin-S~\cite{liu2021swin}  & 219 & 1038  & 47.6/49.5\\
%     ConvNeXt-S~\cite{liu2022convnet}  & 234 & 1027  &\quad-\  /49.6\\
%         \rowcolor{Gray}
%     \textbf{FasterViT-3}  & \textbf{254} & 1076  & \textbf{48.7/49.7}\\
%     \midrule
%     % Focal-S~\citep{yang2021focal}  & 85 & 1130 & 48.0\\
%     Twins-SVT-L~\cite{chu2021twins}  & 164 & -  & 48.8/50.2\\
%     Swin-B~\cite{liu2021swin}  & 172 & 1188  & 48.1/49.7\\
%     ConvNeXt-B~\cite{liu2022convnet}  & 189 & 1170  &\quad-\  /49.9\\
%     \rowcolor{Gray}
%     \textbf{FasterViT-4}  & \textbf{202} & 1290  & \textbf{49.1/50.3}\\
%     \bottomrule

%   \end{tabular}  
%   }
% \caption{Semantic segmentation benchmarks \textbf{ADE20K} dataset~\cite{zhou2017scene} with UPerNet~\cite{xiao2018unified} and pre-trained FasterViT backbones. All model statistics are reported using a input test resolution of $512\times 512$. Throughput is measured in image/sec.}
%     \label{tab:ade_segmentation}
%     % \vspace{-5mm}
% \end{minipage}
% \end{wraptable}
